A Projection Architecture for Dependency Grammar and How it Compares to LFG

This paper explores commonalities and differences between \dachs, a variant of Dependency Grammar, and Lexical-Functional Grammar. \dachs\ is based on traditional linguistic insights, but on modern mathematical tools, aiming to integrate different knowledge systems (from syntax and semantics) via their coupling to an abstract syntactic primitive, the dependency relation. These knowledge systems correspond rather closely to projections in LFG. We will investigate commonalities arising from the usage of the projection approach in both theories, and point out differences due to the incompatible linguistic premises. The main difference to LFG lies in the motivation and status of the dimensions, and the information coded there. We will argue that LFG confounds different information in one projection, preventing it to achieve a good separation of alternatives and calling the motivation of the projection into question.

==> nobi-hyphen.tex <==
\hyphenation{
Hash-funk-tion
Hash-funk-tio-nen
Dis-kurs-wissen
Teil-auf-gabe
beruf-liche
Unifikations-formalis-mus
buch-staben-orien-tierten
an-dere
Sys-tems
Nomina
Allo-morphie
Wort-analysen
aus-gehend
be-deutungs-tragende
Lexikon-organi-sation
Analyse-protokoll
Wort-seman-tik
%re-pr"asentiert
Kombi-nations-regeln
Kate-gorien
De-fini-tion
spe-zielle
% Pr"afixe
Im-ple-men-tation
buch-staben-orien-tiert
Adjektiv-endun-gen
Allo-morph-re-geln
TRUE
Pro-gramm
Kla-ssi-fi-ka-tion
Sprach-ana-lyse-sys-tem
morphem-orientiert
Ana-lyse-pro-gramm
ka-te-go-ri-siert
regexp
Allo-morphe
Lama
Haupt-speicher
dies
Parti-zipI
Para-digma
be-nutzt
}


